Learning continuous models for continuous physics

Dynamical systems that evolve continuously over time are ubiquitous throughout science and engineering. Machine learning (ML) provides data-driven approaches to model and predict the dynamics of such systems. A core issue with this approach is that ML models are typically trained on discrete data, using ML methodologies that are not aware of underlying continuity properties. This results in models that often do not capture any underlying continuous dynamics -- either of the system of interest, or indeed of any related system. To address this challenge, we develop a convergence test based on numerical analysis theory. Our test verifies whether a model has learned a function that accurately approximates an underlying continuous dynamics. Models that fail this test fail to capture relevant dynamics, rendering them of limited utility for many scientific prediction tasks; while models that pass this test enable both better interpolation and better extrapolation in multiple ways. Our results illustrate how principled numerical analysis methods can be coupled with existing ML training/testing methodologies to validate models for science and engineering applications.

==> _s5_conclusions.tex <==

\section{Conclusion}

One of the great challenges in scientific ML is to learn continuous dynamics for physical systems---either ``the'' underlying continuous dynamics, or ``a'' continuous dynamics that leads to good predictive results for the spatial/temporal regime of interest for the ML model---such that the learned ML model can be trusted to give accurate and reliable results.
ML models are trained on discrete points, and typical ML training/testing methodologies are not aware of the continuity properties of the underlying problem from which the data are generated.
Here, we have developed a ContinuousNet methodology, and we showed that convergence (an important criteria used in numerical analysis) can be used for selecting models that have a strong inductive bias towards learning meaningfully continuous dynamics. 
Standard ODE-Net approaches, as well as common SINDy methods, both popular in recent years within the ML community, often do not pass this convergence test.
In contrast, models that pass this ContinuousNet convergence test have favorable properties. 
For instance, models that learned underlying continuous dynamics can be evaluated at lower or higher resolutions. 
%
Our results suggest that principled numerical analysis methods can be coupled with existing ML training/testing methodologies to deliver upon the promise of scientific ML more generally.

Many more concrete directions are of course raised by our methodology.
%
One direction has to do with developing analogous tests to be used for less well-posed dynamical systems.
Such systems are of interest in scientific ML, and such tests will be of greatest interest when one needs to obtain ``the'' correct underlying continuous solution (e.g., to identify correctly qualitative long-term behavior~\cite{ker_disc_cont_92}), rather than ``a'' continuous solution, which is often sufficient for ML prediction tasks.
%
Another direction has to do with whether we can develop analogous tests appropriate for adaptive time-stepping methods, symplectic integrators, and other commonly used numerical simulation methods such as those for optimal control problems using NNs and associated Hamilton-Jacobi partial differential equations~\cite{NGW21,DLM20}.
Work subsequent to the posting of the initial technical report version of this paper has addressed the continuous-discrete equivalence question for learning operators~\cite{BBRMMA23_TR,RMRRBx23_TR}, and likely our ContinuousNet methodology provides a way to operationalize that in practice.
%
A final direction has to do with whether one can obtain strong theoretical results, e.g., ML-style generalization bounds, to guide the use of methods such as these.
Recent theoretical and empirical results suggest that this will be challenging~\cite{MM19_HTSR_ICML,MM20_SDM,MM20a_trends_NatComm,MM21a_simpsons_TR,liam_generaliz_bounds_ICML22}, at least when using traditional approaches to ML-style generalization bounds.
Our success in combining
principled numerical analysis methods with existing ML methodologies also leads one to wonder whether we can use
a posteriori error bound analysis methods to develop practically useful a posteriori generalization bounds for problems such as those we have considered.




==> _s6_extra_misc_nature_comm.tex <==
\paragraph{Competing interests.} The authors declare no competing interests.

\paragraph{Data availability}

The source code for the data generation and models will be made available at \url{https://github.com/a1k12/learning-continuous-physics}.
